Advancements in Arabic Grammatical Error Detection and Correction: An Empirical Investigation

Grammatical error correction (GEC) is a well-explored problem in English with many existing models and datasets. However, research on GEC in morphologically rich languages has been limited due to challenges such as data scarcity and language complexity. In this paper, we present the first results on Arabic GEC using two newly developed Transformer-based pretrained sequence-to-sequence models. We also define the task of multi-class Arabic grammatical error detection (GED) and present the first results on multi-class Arabic GED. We show that using GED information as an auxiliary input in GEC models improves GEC performance across three datasets spanning different genres. Moreover, we also investigate the use of contextual morphological preprocessing in aiding GEC systems. Our models achieve SOTA results on two Arabic GEC shared task datasets and establish a strong benchmark on a recently created dataset. We make our code, data, and pretrained models publicly available.

==> gec_test_results.tex <==

\setlength\dashlinedash{1pt}
\setlength\dashlinegap{1.5pt}


\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lcccc|cccc|cccc|cccc}
    \toprule
    %\cline{1-10}
        \multicolumn{1}{l}{} & \multicolumn{4}{c}{\textbf{QALB-2014}} & \multicolumn{4}{c}{\textbf{QALB-2015-L1}}  & \multicolumn{4}{c}{\textbf{QALB-2015-L2}} & \multicolumn{4}{c}{\textbf{ZAEBUC}} \\
        
        \multicolumn{1}{l}{} & \textbf{P} & \textbf{R} & \textbf{F\textsubscript{1}} & \textbf{F\textsubscript{0.5}} & \textbf{P} & \textbf{R} & \textbf{F\textsubscript{1}} & \textbf{F\textsubscript{0.5}}& \textbf{P} & \textbf{R} & \textbf{F\textsubscript{1}} & \textbf{F\textsubscript{0.5}}& \textbf{P} & \textbf{R} & \textbf{F\textsubscript{1}} & \textbf{F\textsubscript{0.5}}\\\hline

        \textbf{B\&B (2015)} & - & - & - & - & - & - & - & - & 54.1 & 33.3 & 41.2 & 48.1 & - & - & - & -\\
        \textbf{W+ (2018)} & - & - & 70.4 &  - & - & - & 73.2 & - & - & - & - & - & - & - & - & - \\
        \textbf{S+ (2022)} & 79.1 & 65.8 & 71.8 &  76.0 & 78.4 & 70.4 & 74.2 & 76.6 & - & - & - & - & - & - & - & - \\\hline
        
        \textbf{AraBART} & 84.0 &   64.7 &   73.1  &  79.3  &  82.0  &  71.7 &   76.5  & 79.7 &  \textbf{69.6}  & 43.5  & 53.5  & 62.1  & \textbf{86.0}  & 71.6 &  78.2 &  82.7 \\
        \hspace{1em}+Morph & 83.3 &   \textbf{67.4}  &  \textbf{74.5}  &  \textbf{79.5} &   81.7 &   \textbf{73.0}  &  \textbf{77.1} &  79.8 &  68.7 &  43.6 &  53.3 &  61.6 &  85.3  & 71.8 &  78.0  & 82.3 \\
        
        \hspace{1em}+GED\textsuperscript{13} & \textbf{84.1} &  65.0  & 73.3 &  79.4  & 81.5  & 72.7 & 76.8   & 79.5  & 69.3  & \textbf{44.9}  & \textbf{54.5}  & \textbf{62.5} &  85.9  & 73.4  & \textbf{79.2} &  \textbf{83.1}  \\
        \hspace{1em}+Morph+GED\textsuperscript{13} &  83.9  & 65.3  & 73.4  & 79.4  & \textbf{82.6}  & 72.0   & 76.9   & \textbf{80.2}  & 68.2  & 44.8   & 54.1  & 61.8  & 85.2 &  \textbf{73.7}  & 79.0  & 82.6 \\

        \bottomrule
        
    \end{tabular}
\caption{
GEC results on the Test sets of QALB-2014, QALB-2015, and ZAEBUC.
%The best results are bolded.
B\&B (2015), W+ (2018), and S+ (2022) refer to \newcite{bougares-bouamor-2015-ummu}, \newcite{Watson:2018:utilizing}, and \newcite{solyman-etal-2022-automatic}, respectively.
}
\label{tab:gec-test-res}
\end{table*}			

==> gec_test_results_nopnx.tex <==
\setlength\dashlinedash{1pt}
\setlength\dashlinegap{1.5pt}

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lcccc|cccc|cccc|cccc}
    \toprule
    %\cline{1-10}
        \multicolumn{1}{l}{} & \multicolumn{4}{c}{\textbf{QALB-2014}} & \multicolumn{4}{c}{\textbf{QALB-2015-L1}}  & \multicolumn{4}{c}{\textbf{QALB-2015-L2}} & \multicolumn{4}{c}{\textbf{ZAEBUC}} \\

        
        \multicolumn{1}{l}{} & \textbf{P} & \textbf{R} & \textbf{F\textsubscript{1}} & \textbf{F\textsubscript{0.5}} & \textbf{P} & \textbf{R} & \textbf{F\textsubscript{1}} & \textbf{F\textsubscript{0.5}}& \textbf{P} & \textbf{R} & \textbf{F\textsubscript{1}} & \textbf{F\textsubscript{0.5}}& \textbf{P} & \textbf{R} & \textbf{F\textsubscript{1}} & \textbf{F\textsubscript{0.5}}\\\hline

        \textbf{AraBART} & 89.5 &  77.3 &  83.0  & 86.8  & \textbf{90.1}  & 81.4  & 85.5  & 88.2  & \textbf{71.8}  & 40.7  & 52.0 & 62.3  & 89.5  & 76.9  & 82.7  & 86.6 \\
        \hspace{1em}+Morph & 88.4  & 78.9 &  83.4  & 86.3 &  89.9 &  83.1  & 86.4  & \textbf{88.5}  & 70.2  & 41.8  & 52.4  & 61.8 &  88.4   & 76.3 &  81.9  & 85.7 \\
        

        \hspace{1em}+GED\textsuperscript{13} & \textbf{89.8}  & 78.9  & 84.0  & \textbf{87.3}  & 89.8  & 82.2  & 85.8  & 88.2  & 71.0  & 42.8  & \textbf{53.4}  & \textbf{62.7}  & \textbf{89.9}  & 77.8  & \textbf{83.4}  & \textbf{87.2} \\
        
        \hspace{1em}+Morph+GED\textsuperscript{13}  & 88.6  & \textbf{80.0}  & \textbf{84.1}  & 86.7  & 89.8  & \textbf{83.7}  & \textbf{86.6}  & \textbf{88.5}  & 68.9  & \textbf{43.5}  & 53.3  & 61.7  & 88.9  & \textbf{78.4}  & 83.3  & 86.5 \\


        \bottomrule
        


    \end{tabular}
\caption{
No punctuation GEC results on the Test sets of QALB-2014, QALB-2015, and ZAEBUC.
%B\&B (2015) and W+ (2018) refer to \newcite{bougares-bouamor-2015-ummu} and \newcite{Watson:2018:utilizing}, respectively.
}
\label{tab:gec-test-res-nopnx}
\end{table*}



